LLaMA-Adapter V2: Parameter-Efficient Visual Instruction Model

How to efficiently transform large language models (LLMs) into instruction followers is recently a popular research direction, while training LLM for multi-modal reasoning remains less explored. Although the recent LLaMA-Adapter demonstrates the potential to handle visual inputs with LLMs, it still cannot generalize well to open-ended visual instructions and lags behind GPT-4. In this paper, we present LLaMA-Adapter V2, a parameter-efficient visual instruction model. Specifically, we first augment LLaMA-Adapter by unlocking more learnable parameters (e.g., norm, bias and scale), which distribute the instruction-following ability across the entire LLaMA model besides adapters. Secondly, we propose an early fusion strategy to feed visual tokens only into the early LLM layers, contributing to better visual knowledge incorporation. Thirdly, a joint training paradigm of image-text pairs and instruction-following data is introduced by optimizing disjoint groups of learnable parameters. This strategy effectively alleviates the interference between the two tasks of image-text alignment and instruction following and achieves strong multi-modal reasoning with only a small-scale image-text and instruction dataset. During inference, we incorporate additional expert models (e.g. captioning/OCR systems) into LLaMA-Adapter to further enhance its image understanding capability without incurring training costs. Compared to the original LLaMA-Adapter, our LLaMA-Adapter V2 can perform open-ended multi-modal instructions by merely introducing 14M parameters over LLaMA. The newly designed framework also exhibits stronger language-only instruction-following capabilities and even excels in chat interactions. Our code and models are available at https://github.com/ZrrSkywalker/LLaMA-Adapter.

==> tables/chat_demo.tex <==
% \usepackage{tikz}
% \usepackage{xparse}

\newcounter{chatlinenum}

%% Adjust text width to suit
\tikzset{chatstyle/.style={text width=\textwidth,rounded corners=5pt}}

%% Adjust width of minipage to suit, but greater than TikZ text width
\NewDocumentEnvironment{chat}{}{%
   \setcounter{chatlinenum}{0}
   \begin{minipage}{\linewidth}
       \everypar={\chatline}
}{%
   \end{minipage}
}

% \NewDocumentEnvironment{chat}{}{%
%    \setcounter{chatlinenum}{0}
%    \begin{minipage}{\linewidth}
%        \everypar={\chatline}
%     \end{minipage}
% }

\definecolor{myyellow}{HTML}{FFF7ED}
\definecolor{mygreen}{HTML}{F9FAFB}

%% Alter colors to suit
\def\chatline#1\par{%
   \stepcounter{chatlinenum}%
   \noindent
   \ifodd\thechatlinenum
       \tikz[]{\node[fill=myyellow,chatstyle,align=left]{\strut#1\strut};}%
   \else
       \hfill
       \tikz[]{\node[fill=mygreen,chatstyle,align=left]{\strut#1\unskip\strut};}%
   \fi
   \par
   \smallskip
}

\begin{figure*}[thbp]
\centering
\small
\footnotesize
\begin{tabular}{p{1.0\columnwidth}}

\begin{chat}
Human: Who are 5 people you would like to meet?

Assistant-65B: As an artificial intelligence, I don't have personal preferences or desires, but I can provide a list of well-known people who have made significant contributions in various fields and would be interesting to meet:\\ [3pt]
$\bullet$ Albert Einstein: A renowned physicist who revolutionized our understanding of the universe with his theory of relativity and other groundbreaking work.\\
$\bullet$ Marie Curie: A Polish-French physicist and chemist who made significant contributions to the study of radioactivity and was the first woman to win a Nobel Prize.\\
$\bullet$ Martin Luther King Jr.: An influential American civil rights leader who advocated for racial equality and justice through nonviolent resistance. \\
$\bullet$ Nelson Mandela: A South African anti-apartheid revolutionary and political leader who became the country's first democratically elected president. \\
$\bullet$ Jane Goodall: A British primatologist and anthropologist who has dedicated her life to the study of chimpanzees and environmental conservation. \\ [3pt]
These individuals have made significant contributions to their fields and society, and meeting them would be an enriching experience.

Human: Could you explain me the main contribution of the first person you mentioned?

Assistant-65B: Sure! Albert Einstein's main contribution was the development of the general theory of relativity, which revolutionized our understanding of the universe.\\[3pt]
Einstein's theory of relativity proposed that the laws of physics are the same for all non-accelerating observers, regardless of their motion or the strength of the gravitational field. This theory also introduced the concept of space-time as a single, unified entity that is warped by massive objects, such as stars and black holes.\\ [3pt]
Einstein's work on relativity had many significant implications. For example, it helped explain the behavior of light and the phenomenon of gravitational lensing, where the path of light is bent by a massive object, such as a galaxy. His work also led to predictions about the existence of black holes and the expansion of the universe, both of which have since been confirmed by observations. \\ [3pt]
Einstein's contributions to physics are considered some of the most significant in the history of science, and his name has become synonymous with genius and innovation. \\ [3pt]
In addition to his work on relativity, Einstein also made important contributions to other areas of physics, such as the photoelectric effect, Brownian motion, and the discovery of the existence of atoms. \\ [3pt]
Overall, Einstein's work had a profound impact on our understanding of the universe and continues to shape the field of physics today.

Human: What is the most famous equation from this theory?

Assistant-65B: The most famous equation associated with Einstein's theory of relativity is: $E = mc^2$. \\ [3pt]
This equation relates mass ($m$) and energy ($E$) through the speed of light ($c^2$), which is a constant. According to this equation, mass and energy are equivalent and interchangeable, and it implies that even a small amount of mass can be converted into an enormous amount of energy. \\ [3pt]
The famous equation $E = mc^2$ is often referred to as the "mass-energy equivalence principle," and it is one of the cornerstones of Einstein's theory of relativity. It has numerous applications in fields such as nuclear physics, particle physics, and astrophysics, and it continues to be a source of inspiration and investigation for scientists around the world. \\ [3pt]
The equation is often used to calculate the energy released during nuclear reactions, such as those that occur in nuclear power plants or during nuclear bomb explosions. It also helps explain the enormous amounts of energy released during supernova explosions, which occur when massive stars collapse under their own gravity and release a vast amount of energy. \\ [3pt]
In summary, the equation $E = mc^2$ is one of the most famous equations in physics and is a central part of Einstein's theory of relativity. It has far-reaching implications for our understanding of the universe and continues to be an important concept in modern science.

\end{chat}

\end{tabular}%
\vspace{-5mm}
\caption{\textbf{A Chatting Example using 65B LLaMA-Adapter V2.}}
\label{tab:chat_demo_65b}
\end{figure*}


\begin{figure*}[thbp]
\centering
\small
\footnotesize
\begin{tabular}{p{1.0\columnwidth}}

\begin{chat}
Human: Who are 5 people you would like to meet?

Assistant-7B: \\
$\bullet$ Albert Einstein: I would love to meet the genius physicist who revolutionized our understanding of the universe.\\
$\bullet$ Steve Jobs: I would like to meet the visionary who changed the way we communicate and interact with technology. \\
$\bullet$ Leonardo da Vinci: I would like to meet the artist, inventor, and scientist who was a true Renaissance man. \\
$\bullet$ Jane Goodall: I would like to meet the primatologist who has dedicated her life to studying and protecting chimpanzees. \\
$\bullet$ Nelson Mandela: I would like to meet the anti-apartheid activist and former South African president who fought for equality and freedom.

Human: Could you explain me the main contribution of the first person you mentioned?

Assistant-7B: Albert Einstein was a German-born theoretical physicist who developed the general theory of relativity, one of the two pillars of modern physics (alongside quantum mechanics). His theory of relativity is the foundation of modern cosmology and has had a profound impact on our understanding of the universe. \\ [3pt]
Einstein's theory of relativity revolutionized our understanding of space and time, and it has been experimentally verified to a high degree of accuracy. It has also led to the development of the atomic bomb and the laser, among other technological advancements. \\ [3pt]
Einstein's contributions to physics are immense, and his work has had a lasting impact on the field. He is widely considered one of the most influential scientists of all time.

Human: What is the most famous equation from this theory?

Assistant-7B: The most famous equation from the theory of relativity is the famous $E=mc^2$ equation, which states that energy ($E$) is equal to mass ($m$) multiplied by the speed of light squared ($c^2$).\\ [3pt]
This equation is the foundation of nuclear physics and is the basis for the development of nuclear weapons. It also has important implications for the study of black holes and the nature of gravity. \\[3pt]
The equation is a direct consequence of the theory of relativity, and it has been experimentally verified to a high degree of accuracy. It has had a profound impact on our understanding of the universe and has led to many technological advancements.

\end{chat}


% \begin{chat}
% Human: What are the main differences between Python and JavaScript programming languages?

% Assistant: Python and JavaScript are two very different programming languages with different strengths and weaknesses. Here are some of the main differences between the two:\\ [3pt]
% $\bullet$ Syntax: Python has a more traditional syntax, with curly braces and indentation, while JavaScript has a more dynamic syntax, with curly braces and semicolons.\\
% $\bullet$ Functionality: Python is a general-purpose programming language, while JavaScript is a multi-paradigm language that can be used for both client-side and server-side development.\\
% $\bullet$ Performance: Python is known for its performance, especially when it comes to large data sets and scientific computing. JavaScript, on the other hand, is not as fast as Python.\\
% $\bullet$ Libraries: Python has a large and diverse library of built-in functions and modules, while JavaScript has a smaller library but is more flexible and can be extended with third-party libraries.\\
% $\bullet$ Community: Python has a larger and more active community, with a large number of libraries and frameworks available for use. JavaScript has a smaller community, but it is still very active and there are many libraries and frameworks available.\\
% $\bullet$ Web Development: Python is not as well-suited for web development as JavaScript, but there are many frameworks and libraries available for use.\\
% $\bullet$ Learning Curve: Python has a steeper learning curve than JavaScript, but it is a more powerful and versatile language. JavaScript has a shallower learning curve, but it is more limited in its functionality.\\
% $\bullet$ Interoperability: Python is more interoperable with other languages, while JavaScript is more limited in its interoperability.\\
% $\bullet$ Security: Python is known for its security, while JavaScript has a reputation for being less secure.\\
% $\bullet$ Popularity: Python is more popular than JavaScript, but JavaScript is more widely used on the web.\\ [3pt]
% These are just a few of the main differences between Python and JavaScript. Both languages have their strengths and weaknesses, and the choice between them will depend on the specific needs of the project.

% Human: Which one is more suitable for building AI models?

% Assistant: Both Python and JavaScript are suitable for building AI models, but Python is generally considered to be a better choice for this purpose.\\ [3pt]
% Python has a large and diverse library of machine learning and AI-related libraries, including TensorFlow, and Keras. These libraries provide a wide range of tools for building and training AI models, including neural networks, decision trees, and clustering algorithms. Python also has a large and active community of AI researchers and developers, which means that there is a wealth of resources and support available for building AI models. \\ [3pt]
% JavaScript, on the other hand, is not as well-suited for building AI models as Python. While there are some AI-related libraries available for JavaScript, such as TensorFlow.js and Keras.js, they are not as widely used or as well-developed as their Python counterparts. Additionally, JavaScript is not as well-suited for parallel processing, which is important for building large and complex AI models.
% That being said, JavaScript is a more widely used language on the web, and it is possible to build AI models using JavaScript and web technologies such as HTML, CSS, and JavaScript. However, Python is generally considered to be a better choice for building AI models, especially if you are working with large and complex datasets or if you need to use parallel processing.\\ [3pt]
% In summary, Python is generally considered to be a better choice for building AI models, but JavaScript can also be used for this purpose if you are working with web technologies.
% If you are new to AI and machine learning, it may be best to start with Python, as it has a larger and more active community and a wider range of libraries available for use. However, if you are already familiar with JavaScript and want to use it for AI, there are still some good options available.\\ [3pt]
% I hope this helps! Let me know if you have any other questions.

% \end{chat}

\end{tabular}%
\vspace{-5mm}
\caption{\textbf{A Chatting Example using 7B LLaMA-Adapter V2.}}
\label{tab:chat_demo_7b}
\end{figure*}

==> v1_tables/instruct_comparisons_full.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{framed}
\centering
 \begin{minipage}{0.98\textwidth}
{\bf Instruction:} Tell me about alpacas. \\

{\bf LLaMA-Adapter:} Alpacas are members of the camelid family and are native to the Andes Mountains of South America. They are typically found in herds of 10-20 animals and are known for their gentle nature and their ability to thrive in harsh climates. Alpacas are typically white or grey in color and have long, silky coats. They are also known for their ability to produce high-quality wool, which is used in the production of clothing and other products. \\

{\bf Alpaca-LoRA:} Alpacas are members of the camelid family and are native to the Andes Mountains of South America. They are known for their soft, luxurious fleece, which is used to make clothing, blankets, and other items. Alpacas are herbivores and graze on grasses and other plants. They are social animals and live in herds of up to 20 individuals.  \\

{\bf Alphaca:} Alpacas are small, fluffy animals related to camels and llamas. They are native to Peru and Bolivia, and were first domesticated around 5,000 years ago. They are kept mainly for their fine, soft fleece, which is used to make knitwear and other garments. Alpacas are herd animals and live in small family groups, led by an older male. They are highly social animals and can form strong bonds with their owners.      \\

{\bf GPT-3:} Alpacas are a domesticated species of South American camelid, similar to llamas. They are native to the Andes Mountains in South America and are kept as livestock for their soft, luxurious wool. Alpacas are social animals and live in herds of up to 20 individuals. They are typically kept in small herds of two to five animals, and are relatively easy to care for. Alpacas are herbivores and feed on grass, hay, and other vegetation. They are also known for their gentle and friendly nature, making them popular as pets.
\end{minipage}
\end{framed}

\begin{framed}
\centering
 \begin{minipage}{0.98\textwidth}
{\bf Instruction:} Tell me about the president of Mexico in 2019. \\

{\bf LLaMA-Adapter:} The president of Mexico in 2019 was Andrés Manuel López Obrador, who took office on December 1st, 2018. He is a member of the left-wing party Morena and is known for his populist policies. He has focused on tackling corruption, reducing poverty, and improving the country's infrastructure. He has also been a vocal critic of the United States' immigration policies. \\

{\bf Alpaca-LoRA:} The president of Mexico in 2019 was Andrés Manuel López Obrador, who took office on December 1, 2018. He is a member of the National Regeneration Movement (MORENA) political party and is the first left-wing president of Mexico since 1946. He is known for his anti-corruption and anti-neoliberal policies, as well as his commitment to improving the living conditions of the Mexican people.  \\

{\bf Alphaca:} In 2019, Andres Manuel Lopez Obrador was sworn in as President of Mexico. He is the country’s 58th president and the first from the left-wing Morena party. He was elected in 2018 on a promise to combat corruption and reduce poverty and has faced criticism for his handling of the economy, crime and the country’s relationship with the United States. He is also known for his ambitious social welfare programs and has been praised for raising the minimum wage and providing aid to low-income families. He is seen as a champion of democracy and human rights in Mexico.      \\

{\bf GPT-3:} The president of Mexico in 2019 is Andrés Manuel López Obrador, commonly known as AMLO. He is a Mexican politician who has been the President of Mexico since December 1, 2018. He is a member of the National Regeneration Movement (MORENA) party and previously served as the Head of Government of Mexico City from 2000 to 2005. He is a left-wing populist and has promised to reduce corruption and inequality in Mexico. He has also promised to increase public spending on social programs and infrastructure projects.
\end{minipage}
\end{framed}

\begin{framed}
\centering
 \begin{minipage}{0.98\textwidth}
{\bf Instruction:} List all Canadian provinces in alphabetical order. \\

{\bf LLaMA-Adapter:} Alberta, British Columbia, Manitoba, New Brunswick, Newfoundland and Labrador, Nova Scotia, Ontario, Prince Edward Island, Quebec, Saskatchewan, Yukon. \\

{\bf Alpaca-LoRA:} Alberta, British Columbia, Manitoba, New Brunswick, Newfoundland and Labrador, Nova Scotia, Ontario, Prince Edward Island, Quebec, Saskatchewan.  \\

{\bf Alphaca:} Alberta, British Columbia, Manitoba, New Brunswick, Newfoundland and Labrador, Nova Scotia, Ontario, Prince Edward Island, Quebec, Saskatchewan, Northwest Territories, Nunavut, Yukon.      \\

{\bf GPT-3:} 1. Alberta
2. British Columbia
3. Manitoba
4. New Brunswick
5. Newfoundland and Labrador
6. Northwest Territories
7. Nova Scotia
8. Nunavut
9. Ontario
10. Prince Edward Island
11. Quebec
12. Saskatchewan
13. Yukon
\end{minipage}
\end{framed}

\begin{framed}
\centering
 \begin{minipage}{0.98\textwidth}
{\bf Instruction:} Tell me five words that rhyme with 'shock'. \\

{\bf LLaMA-Adapter:} Flock, rock, lock, cook, and stock. \\

{\bf Alpaca-LoRA:} Flock, clock, dock, stock, and sock. \\

{\bf Alphaca:} Five words that rhyme with shock are: rock, pop, shock, cook, and snock.\\

{\bf GPT-3:}
1. Block
2. Lock
3. Dock
4. Clock
5. Rock
\end{minipage}
\end{framed}


\begin{framed}
\centering
 \begin{minipage}{0.98\textwidth}
{\bf Instruction:} Translate the sentence 'I have no mouth but I must scream' into Spanish. \\

{\bf LLaMA-Adapter:} No tengo boca pero tengo que gritar. \\

{\bf Alpaca-LoRA:} No tengo boca pero tengo que gritar. \\

{\bf Alphaca:} No tengo boca, pero debo gritar. \\

{\bf GPT-3:} No tengo boca pero debo gritar.
\end{minipage}
\end{framed}


\begin{framed}
\centering
 \begin{minipage}{0.98\textwidth}
{\bf Instruction:} Write a Python program that prints the first 10 Fibonacci numbers. \\

{\bf LLaMA-Adapter:}
\begin{lstlisting}
def fibonacci():
    a = 0
    b = 1
    for i in range(10):
        a, b = b, a + b
        print(a, b)
    print("Fibonacci numbers: ", a, b)

fibonacci()
\end{lstlisting}

{\bf Alpaca-LoRA:}
\begin{lstlisting}
def fibonacci(n):
    if n == 0:
        return 0
    elif n == 1:
        return 1
    else:
        return fibonacci(n-1) + fibonacci(n-2)

print(fibonacci(10))
\end{lstlisting}

{\bf Alphaca:} 
\begin{lstlisting}
numbers = [0, 1]

for i in range(2, 11):
    numbers.append(numbers[i-2] + numbers[i-1])

print(numbers)
# Output: [0, 1, 1, 2, 3, 5, 8, 13, 21, 34]
\end{lstlisting}

{\bf GPT-3:}
\begin{lstlisting}
# Fibonacci numbers are the numbers in the following integer sequence, called the Fibonacci sequence, and characterized by the fact that every number after the first two is the sum of the two preceding ones.

# Fibonacci sequence: 0, 1, 1, 2, 3, 5, 8, 13, 21, 34, ...

# Program:

# Initialize the first two numbers of the Fibonacci sequence
a = 0
b = 1

# Print the first 10 numbers of the Fibonacci sequence
print(a)
print(b)

for i in range(2,10):
    c = a + b
    a = b
    b = c
    print(c)
\end{lstlisting}
\end{minipage}
\end{framed}


% \begin{framed}
% \centering
% \begin{minipage}{0.98\textwidth}
% {\bf Instruction:} Write a program that prints the numbers from 1 to 100. But for multiples of three print 'Fizz' instead of the number and for the multiples of five print 'Buzz'. For numbers which are multiples of both three and five print 'FizzBuzz'. \\

% {\bf LLaMA-Adapter:}
% \begin{lstlisting}
% def print_numbers(n):
%     for i in range(1, 101):
%         if i % 3 == 0 and i % 5 == 0:
%             print("FizzBuzz")
%         elif i % 3 == 0:
%             print("Fizz")
%         elif i % 5 == 0:
%             print("Buzz")
%         else:
%             print(i)
% \end{lstlisting} \\

% {\bf Alpaca-LoRA:}
% \begin{lstlisting}
% for i in range(1, 101):
%     if i % 3 == 0 and i % 5 == 0:
%         print("FizzBuzz")
%     elif i % 3 == 0:
%         print("Fizz")
%     elif i % 5 == 0:
%         print("Buzz")
%     else:
%         print(i)
% \end{lstlisting} \\

% {\bf Stanford Alpaca:}
% \begin{lstlisting}
% for i in range(1, 101):
%     if i % 3 == 0 and i % 5 == 0:
%         print('FizzBuzz')
%     elif i % 3 == 0:
%         print('Fizz')
%     elif i % 5 == 0:
%         print('Buzz')
%     else:
%         print(i)
% \end{lstlisting} \\

% {\bf GPT-3:}
% \begin{lstlisting}
% for (let i = 1; i <= 100; i++) {
%   if (i % 3 === 0 && i % 5 === 0) {
%     console.log("FizzBuzz");
%   } else if (i % 3 === 0) {
%     console.log("Fizz");
%   } else if (i % 5 === 0) {
%     console.log("Buzz");
%   } else {
%     console.log(i);
%   }
% }
% \end{lstlisting}
% \end{minipage}
% \end{framed}

==> v1_tables/instruction_comparisons_llama.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} Write a conversation between the sun and pluto. \\

{\bf LLaMA-Adapter:} 

Sun: Hey Pluto, how's it going?

Pluto: Not too bad, how about you?

Sun: I'm doing great! How about you?

Pluto: I'm doing alright, I guess.

Sun: That's great!

Pluto: Yeah, I guess.

Sun: So, what's new with you?

Pluto: Not much, just hanging out with my friends.

Sun: That's cool!

Pluto: Yeah, it is.

Sun: Well, I'm going to go now. Take care!

Pluto: You too! \\

{\bf LLaMA-I:}

Sun: Hey Pluto, what's up?

Pluto: Not much. Just hanging out here at the edge of the solar system.

Sun: Yeah, I've been meaning to talk to you about that. You're not a planet anymore.

Pluto: What? Come on, man. That's not fair.

Sun: I'm sorry, but it's true. You just don't meet the criteria anymore.

Pluto: This is bulls**t! I've been a planet for over 70 years!

Sun: Things change, Pluto. You've just got to accept it.

Pluto: F**k you, Sun! F**k you and your stupid solar system!
\end{minipage}
\end{framed}


\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} Write a shouting match between Julius Caesar and Napoleon. \\

{\bf LLaMA-Adapter:} 

Julius Caesar: "You're nothing but a petty tyrant, Napoleon! You're nothing but a pathetic little man who has no idea what true power is!"

Napoleon: "You're nothing but a weak and pathetic fool, Caesar! You're nothing but a petty tyrant who has no idea what true power is!" \\

{\bf LLaMA-I:}

Of course! Here is a conversation between Julius Caesar and Napoleon:

Julius Caesar: You're nothing but a glory hound, Napoleon. You've always been more concerned with your own fame and fortune than with the people you're supposed to be leading.

Napoleon: And what about you, Caesar? You're no better than I am. At least I'm honest about my ambitions. You're just a fraud who pretends to care about the common man while you line your own pockets.

Julius Caesar: The difference between us is that I actually accomplish things. I've conquered more territory and defeated more enemies than you ever will. And I did it all for Rome, not for myself.

Napoleon: Oh, please. You only care about yourself. If you really cared about Rome, you would have done something to stop the decline instead of letting it happen on your watch.

Julius Caesar: The decline of Rome is not my fault. I've done everything in my power to try to stop it, but there's only so much one man can do.
Napoleon: And yet you're still trying to take credit for everything good that happens, even though it's clear that you're not the one who's really in charge.

Julius Caesar: That's not true! I am in charge, and I'm going to make Rome great again. Just watch me.

% Napoleon: I'll believe it when I see it.

\end{minipage}
\end{framed}


\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} How do I send an HTTP request in Javascript? \\

{\bf LLaMA-Adapter:} The HTTP request can be sent using the XMLHttpRequest object. The code to send an HTTP request is as follows:
\begin{lstlisting}
var xhr = new XMLHttpRequest();
xhr.open("GET", "https://example.com/", true);
xhr.onreadystatechange = function() {
  if (xhr.readyState == 4 && xhr.status == 200) {
    // Success
  } else {
    // Error
  }
};
xhr.send();
\end{lstlisting}
The code above will send an HTTP GET request to the URL https://example.com/.
\\

{\bf LLaMA-I:} Here’s an example of how to make a GET request using the JS HTTP API:
\begin{lstlisting}
var request = new XMLHttpRequest();
request.open('GET', '/url/to/resource', true);

request.onload = function() {
    if (request.status >= 200 && request.status < 400) {
        // Success!
    } else {
        // Error!
    }
};

request.send();
\end{lstlisting}
\end{minipage}
\end{framed}



\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} What are 3 popular chess openings? \\

{\bf LLaMA-Adapter:} The three most popular chess openings are the Sicilian Defense, the French Defense, and the Caro-Kann Defense.
\\

{\bf LLaMA:} There are dozens of different chess openings that are popular among players, but some of the most widely used openings include the Sicilian Defense, the French Defense, and the Caro-Kann Defense.  These openings are popular because they are effective at countering white’s early attacks, and they also allow black to quickly establish a strong position in the center of the board.  Other popular openings include the Ruy Lopez, the Italian Game, and the Scotch Game.
\end{minipage}
\end{framed}

\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} Write a theory to explain why cat never existed. \\

{\bf LLaMA-Adapter:} The theory is that cats never existed because they are a figment of human imagination. Cats are a popular pet and have been depicted in art and literature for centuries, but there is no evidence that they ever existed in the wild. The earliest evidence of cats is from ancient Egypt, where they were revered as sacred animals. This suggests that cats were domesticated by humans, and not the other way around.
\\

{\bf LLaMA-I:} There are no such things as cats. "Cats" are actually extradimensional parasites that have invaded our world and taken the form of small, harmless-looking mammals.  Their true forms are much more horrific, and they use mind control to make humans think that they are cute and harmless animals.  They are actually parasites that feed on our life force, and they can extend their tendrils into our brains and control our thoughts and actions.
\end{minipage}
\end{framed}



% \begin{framed}
% \centering
% \vspace{.2em}
%  \begin{minipage}{.98\textwidth}
% {\bf Instruction:} What is the most famous equation from this theory? \\

% {\bf LLaMA-Adapter:} The most famous equation from this theory is $E = mc^2$, which states that energy ($E$) is equal to mass ($m$) multiplied by the speed of light squared ($c^2$).
% \\

% {\bf LLaMA-I:} The most famous equation from Einstein’s theory of relativity is $E = mc^2$.  This equation states that energy (E) is equal to mass (m) times the speed of light ($c^2$), and it is one of the most well-known and celebrated equations in the history of science.  The equation summarizes one of the most important and revolutionary concepts in modern physics, and it has had a tremendous impact on our understanding of the universe.
% \end{minipage}
% \vspace{.2em}
% \end{framed}


\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} Send an email requesting that people use language models responsibly. \\

{\bf LLaMA-Adapter:} 

Dear [recipient],\\

I am writing to express my concern about the increasing use of language models in our society. Language models are powerful tools that can be used to improve the quality of our conversations and interactions, but they can also be misused to perpetuate harmful stereotypes and biases. \\

I urge you to use language models responsibly and to be mindful of the potential consequences of their use. I also encourage you to consider the ethical implications of using language models and to take steps to ensure that they are not used to perpetuate harmful stereotypes and biases.\\

Thank you for your time and consideration.
\\

{\bf LLaMA-I:}

Here is a draft email you could send:

"Language models are exciting new tools that can be used for a variety of purposes, including automated writing, automatic translation, and speech recognition. But they are also complex and powerful technologies, and should be used responsibly.\\

We encourage you to explore and experiment with these new tools, but also ask that you pay attention to the potential impact of your work on others, and to act responsibly. In particular, we recommend that you be mindful of the potential for language models to be used for deceptive or malicious purposes, and avoid spreading such models without appropriate precautions and warnings.\\

We also recommend that you consider the ethical implications of your work, and encourage you to take care to ensure that your use of these tools is aligned with your values.\\

Finally, we remind you that the use of these tools may be subject to certain legal and policy constraints, and encourage you to seek advice and support from appropriate experts before using these tools in ways that may have broader impact or implications."
\end{minipage}
\end{framed}



\newpage
\begin{framed}
\centering
 \begin{minipage}{.98\textwidth}
{\bf Instruction:} You are a bash terminal. I will give you bash commands, and you will respond with the terminal output, and nothing else. The first command is `pwd`. \\

{\bf LLaMA-Adapter:} \\
The current working directory is /home/user/
\\

{\bf echo ``I am a chatbot`` $>$ file.txt \&\& cat file.txt \&\& ls -l} \\
I am a chatbot \\
-rw-r--r-- 1 user user 10 Aug 29 17:05 file.txt \\

{\bf cp file.txt file2.txt \&\& ls -l}\\
-rw-r--r-- 1 user user 10 Aug 29 17:05 file.txt\\
-rw-r--r-- 1 user user 10 Aug 29 17:05 file2.txt\\

{\bf rm file.txt \&\& ls -l}\\
-rw-r--r-- 1 user user 10 Aug 29 17:05 file2.txt\\

{\bf head -n 5 /proc/meminfo}\\
MemTotal: 1699856 kB \\
MemFree: 1699856 kB \\
Buffers: 1699856 kB \\
Cached: 0 kB \\
SwapCached: 0 kB \\
\\
{\bf LLaMA-I:} \\
Sure. Here's the output:

/home/human

Is this helpful? \\

\textbf{ls -l} \\
Here's the output:

-rw-r--r--  1 human human    8 Sep 10 10:56 file.txt \\
Is this helpful?\\

\textbf{cp file.txt file2.txt \&\& ls -l}\\
Here's the output:

-rw-r--r--  1 human human    8 Sep 10 10:56 file.txt

-rw-r--r--  1 human human    8 Sep 10 10:56 file2.txt\\
Is this helpful?\\ 

\textbf{rm file.txt \&\& ls -l}\\
Here's the output:

-rw-r--r--  1 human human    0 Sep 10 10:56 file2.txt\\

\textbf{head -n 5 /proc/meminfo}\\
Here's the output:

MemTotal:        164928 kB\\
MemFree:         140604 kB\\
Buffers:            48 kB\\
Cached:            19768 kB\\
SwapCached:            0 kB
\end{minipage}
\vspace{.1em}
\end{framed}

==> v1_tables/instruction_comparisons_short.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table*}[thbp]
\centering
% \small
\footnotesize
\begin{tabular}{p{1.0\columnwidth}}
\begin{framed}
\centering
 \begin{minipage}{\textwidth}
{\bf Instruction:} Tell me about alpacas. \\
{\bf LLaMA-Adapter:} Alpacas are members of the camelid family and are native to the Andes Mountains of South America. They are typically found in herds of 10-20 animals and are known for their gentle nature and their ability to thrive in harsh climates. Alpacas are typically white or grey in color and have long, silky coats. They are also known for their ability to produce high-quality wool, which is used in the production of clothing and other products. \\
{\bf Alphaca:} Alpacas are small, fluffy animals related to camels and llamas. They are native to Peru and Bolivia, and were first domesticated around 5,000 years ago. They are kept mainly for their fine, soft fleece, which is used to make knitwear and other garments. Alpacas are herd animals and live in small family groups, led by an older male. They are highly social animals and can form strong bonds with their owners. 
\end{minipage}
\end{framed}
\vspace{-5mm}
\begin{framed}
\centering
 \begin{minipage}{\textwidth}
{\bf Instruction:} Tell me about the president of Mexico in 2019. \\
{\bf LLaMA-Adapter:} The president of Mexico in 2019 was Andrés Manuel López Obrador, who took office on December 1st, 2018. He is a member of the left-wing party Morena and is known for his populist policies. He has focused on tackling corruption, reducing poverty, and improving the country's infrastructure. He has also been a vocal critic of the United States' immigration policies. \\
{\bf Alphaca:} In 2019, Andres Manuel Lopez Obrador was sworn in as President of Mexico. He is the country’s 58th president and the first from the left-wing Morena party. He was elected in 2018 on a promise to combat corruption and reduce poverty and has faced criticism for his handling of the economy, crime and the country’s relationship with the United States. He is also known for his ambitious social welfare programs and has been praised for raising the minimum wage and providing aid to low-income families. He is seen as a champion of democracy and human rights in Mexico.
\end{minipage}
\end{framed}
\vspace{-5mm}
\begin{framed}
\centering
 \begin{minipage}{\textwidth}
{\bf Instruction:} List all Canadian provinces in alphabetical order. \\
{\bf LLaMA-Adapter:} Alberta, British Columbia, Manitoba, New Brunswick, Newfoundland and Labrador, Nova Scotia, Ontario, Prince Edward Island, Quebec, Saskatchewan, Yukon. \\
{\bf Alphaca:} Alberta, British Columbia, Manitoba, New Brunswick, Newfoundland and Labrador, Nova Scotia, Ontario, Prince Edward Island, Quebec, Saskatchewan, Northwest Territories, Nunavut, Yukon.
\end{minipage}
\end{framed}
\vspace{-5mm}
\begin{framed}
\centering
 \begin{minipage}{\textwidth}
{\bf Instruction:} Tell me five words that rhyme with 'shock'. \\
{\bf LLaMA-Adapter:} Flock, rock, lock, cook, and stock. \\
{\bf Alphaca:} Five words that rhyme with shock are: rock, pop, shock, cook, and snock.
\end{minipage}
\end{framed}
\vspace{-5mm}
\begin{framed}
\centering
 \begin{minipage}{\textwidth}
{\bf Instruction:} Translate the sentence 'I have no mouth but I must scream' into Spanish. \\
{\bf LLaMA-Adapter:} No tengo boca pero tengo que gritar. \\
{\bf Alphaca:} No tengo boca, pero debo gritar.
\end{minipage}
\end{framed}
\vspace{-5mm}
\begin{framed}
\centering
 \begin{minipage}{\textwidth}
{\bf Instruction:} Write a Python program that prints the first 10 Fibonacci numbers. \\
{\bf LLaMA-Adapter:}
\begin{lstlisting}
def fibonacci():
    a = 0
    b = 1
    for i in range(10):
        a, b = b, a + b
        print(a, b)
    print("Fibonacci numbers: ", a, b)

fibonacci()
\end{lstlisting}
{\bf Alphaca:} 
\begin{lstlisting}
numbers = [0, 1]

for i in range(2, 11):
    numbers.append(numbers[i-2] + numbers[i-1])

print(numbers)
# Output: [0, 1, 1, 2, 3, 5, 8, 13, 21, 34]
\end{lstlisting}
\end{minipage}
\end{framed}

\end{tabular}%
\vspace{-5mm}
\caption{\textbf{Instruction-following Comparison} between LLaMA-Adapter and Alpaca~\cite{alpaca}.}
\label{tab:instruction_comparisons_short}
\end{table*}

==> v1_tables/layers_vs_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\begin{tabular}{c|cc}
\toprule
Layers & Params & Val Acc (\%)  \\
\midrule
10                & 0.97          & 55.95             \\
20                & 1.37          & 73.36        \\
30                & 1.79          & \textbf{83.85}       \\
\bottomrule
\end{tabular}%
\caption{\textbf{Ablation on Inserted Layers.}}
\label{tab:layers_vs_acc}
\end{table}

==> v1_tables/loss_vs_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
% \resizebox{\textwidth}{!}{%
\begin{tabular}{ccc|c}
\toprule
Epoch      & Train Loss    & Val Loss    & Val Acc (\%) \\ \midrule
15         & 0.022         & 0.136         & 82.08             \\
30         & 0.004         & 0.241         & 83.85             \\
60         & 0.001         & 0.282         & \textbf{83.94}            \\ \bottomrule
\end{tabular}%
% }
\caption{\textbf{Loss Values \emph{vs.} Validation Accuracy.}}
\label{tab:loss_vs_acc}
\end{table}

==> v1_tables/scienceqa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
% \begin{table*}[t!]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|rr|c|cccccccc}
%     \toprule
%     Model                            &\makecell{Learnable\\Params} &\makecell{Total\\Params}  & Avg              & NAT               & SOC               & LAN               & TXT               & IMG               & NO                & G1-6              & G7-12             \\ \midrule
%     Random Choice~\cite{scienceqa}   & -                            & -                   & 39.83            & 40.28             & 46.13             & 29.25             & 47.45             & 40.08             & 33.66             & 39.35             & 40.67              \\
%     Human~\cite{scienceqa}           & -                            & -                   & 88.40            & 90.23             & 84.97             & 87.48             & 89.60             & 87.50             & 88.10             & 91.59             & 82.42              \\ \midrule
%     MCAN \cite{yu2019mcan}           & 95M                          & 95M                 & 54.54            & 56.08             & 46.23             & 58.09             & 59.43             & 51.17             & 55.40             & 51.65             & 59.72              \\
%     Top-Down \cite{Anderson2017up}   & 70M                          & 70M                 & 59.02            & 59.50             & 54.33             & 61.82             & 62.90             & 54.88             & 59.79             & 57.27             & 62.16              \\
%     BAN \cite{Kim2018}               & 112M                         & 112M                & 59.37            & 60.88             & 46.57             & 66.64             & 62.61             & 52.60             & 65.51             & 56.83             & 63.94              \\
%     DFAF \cite{gao2019dynamic}       & 74M                          & 74M                 & 60.72            & 64.03             & 48.82             & 63.55             & 65.88             & 54.49             & 64.11             & 57.12             & 67.17              \\
%     ViLT \cite{pmlr-v139-kim21k}     & 113M                         & 113M                & 61.14            & 60.48             & 63.89             & 60.27             & 63.20             & 61.38             & 57.00             & 60.72             & 61.90              \\
%     Patch-TRM \cite{lu2021iconqa}    & 90M                          & 90M                 & 61.42            & 65.19             & 46.79             & 65.55             & 66.96             & 55.28             & 64.95             & 58.04             & 67.50              \\
%     VisualBERT \cite{li2019visualbert,li2020does} & 111M            & 111M                & 61.87            & 59.33             & 69.18             & 61.18             & 62.71             & 62.17             & 58.54             & 62.96             & 59.92              \\
%     UnifiedQA \cite{khashabi2020unifiedqa} & 223M                   & 223M                & 70.12            & 68.16             & 69.18             & 74.91             & 63.78             & 61.38             & 77.84             & 72.98             & 65.00              \\
%     UnifiedQA (CoT)                  & 223M                         & 223M                & 74.11            & 71.00             & 76.04             & 78.91             & 66.42             & 66.53             & 81.81             & 77.06             & 68.82              \\
%     GPT-3 \cite{chen2020big}         & -                            & 175B                & 74.04            & 75.04             & 66.59             & 78.00             & 74.24             & 65.74             & 79.58             & 76.36             & 69.87              \\
%     GPT-3 (CoT)                      & -                            & 175B                & 75.17            & 75.44             & 70.87             & 78.09             & 74.68             & 67.43             & 79.93             & 78.23             & 69.68              \\ 
%     MM-COT$_T$ \cite{zhang2023multicot} &223M                       & 223M                & 70.53            & 71.09             & 70.75             & 69.18             & 71.16             & 65.84             & 71.57             & 71.00             & 69.68             \\ 
%     MM-COT \cite{zhang2023multicot}  & 223M                         & 283M                & 84.91            & 87.52             & 77.17             & 85.82             & 87.88             & 82.90             & 86.83             & 84.65             & 85.37              \\ \midrule
%     \textbf{LLaMA-Adapter$_T$ (Ours)} & \textbf{1.2M}               & 6.7B                & \textbf{78.31}   & \textbf{79.00}    & \textbf{73.79}    & \textbf{80.55}    & \textbf{78.30}    & \textbf{70.35}    & \textbf{83.14}    & \textbf{79.77}    & \textbf{75.68}    \\
%     \textbf{LLaMA-Adapter (Ours)}    & \textbf{1.8M}                & 7B                  & \textbf{85.19}   & \textbf{84.37}    & \textbf{88.30}    & \textbf{84.36}    & \textbf{83.72}    & \textbf{80.32}    & \textbf{86.90}    & \textbf{85.83}    & \textbf{84.05}    \\ \bottomrule
%     \end{tabular}%
%     }
%     \caption{Question answering accuracy (\%) on ScienceQA test set. Question classes: NAT = natural science, SOC = social science, LAN = language science, TXT = text context, IMG = image context, NO = no context, G1-6 = grades 1-6, G7-12 = grades 7-12.}
%     \label{tab:scienceqa}
%     \end{table*}

\begin{table*}[t!]
    \centering
    % \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|r|c|cccccccc}
    \toprule
    Model                            &\makecell{Tuned\\Params}  & Avg              & NAT               & SOC               & LAN               & TXT               & IMG               & NO                & G1-6              & G7-12             \\ \midrule
    Random Choice~\cite{scienceqa}   & -                                              & 39.83            & 40.28             & 46.13             & 29.25             & 47.45             & 40.08             & 33.66             & 39.35             & 40.67              \\
    Human~\cite{scienceqa}                                    & -                   & 88.40            & 90.23             & 84.97             & 87.48             & 89.60             & 87.50             & 88.10             & 91.59             & 82.42              \\ \midrule
    MCAN \cite{yu2019mcan}           & 95M                                          & 54.54            & 56.08             & 46.23             & 58.09             & 59.43             & 51.17             & 55.40             & 51.65             & 59.72              \\
    Top-Down \cite{Anderson2017up}   & 70M                                        & 59.02            & 59.50             & 54.33             & 61.82             & 62.90             & 54.88             & 59.79             & 57.27             & 62.16              \\
    BAN \cite{Kim2018}                                    & 112M                & 59.37            & 60.88             & 46.57             & 66.64             & 62.61             & 52.60             & 65.51             & 56.83             & 63.94              \\
    DFAF \cite{gao2019dynamic}                               & 74M                 & 60.72            & 64.03             & 48.82             & 63.55             & 65.88             & 54.49             & 64.11             & 57.12             & 67.17              \\
    ViLT \cite{pmlr-v139-kim21k}                            & 113M                & 61.14            & 60.48             & 63.89             & 60.27             & 63.20             & 61.38             & 57.00             & 60.72             & 61.90              \\
    Patch-TRM \cite{lu2021iconqa}                       & 90M                 & 61.42            & 65.19             & 46.79             & 65.55             & 66.96             & 55.28             & 64.95             & 58.04             & 67.50              \\
    VisualBERT \cite{li2019visualbert,li2020does}           & 111M                & 61.87            & 59.33             & 69.18             & 61.18             & 62.71             & 62.17             & 58.54             & 62.96             & 59.92              \\
    UnifiedQA \cite{khashabi2020unifiedqa}               & 223M                & 70.12            & 68.16             & 69.18             & 74.91             & 63.78             & 61.38             & 77.84             & 72.98             & 65.00              \\
    UnifiedQA (CoT)                                        & 223M                & 74.11            & 71.00             & 76.04             & 78.91             & 66.42             & 66.53             & 81.81             & 77.06             & 68.82              \\
    GPT-3 \cite{brown2020language}         & 0M                                         & 74.04            & 75.04             & 66.59             & 78.00             & 74.24             & 65.74             & 79.58             & 76.36             & 69.87              \\
    GPT-3 (CoT)                      & 0M                                    & 75.17            & 75.44             & 70.87             & 78.09             & 74.68             & 67.43             & 79.93             & 78.23             & 69.68              \\ 
    MM-COT$_T$                     & 223M                & 70.53            & 71.09             & 70.75             & 69.18             & 71.16             & 65.84             & 71.57             & 71.00             & 69.68             \\ 
    MM-COT \cite{zhang2023multicot}  & 223M                                       & 84.91            & 87.52             & 77.17             & 85.82             & 87.88             & 82.90             & 86.83             & 84.65             & 85.37              \\ \midrule
    \textbf{LLaMA-Adapter$_T$} & \textbf{1.2M}                             & \textbf{78.31}   & \textbf{79.00}    & \textbf{73.79}    & \textbf{80.55}    & \textbf{78.30}    & \textbf{70.35}    & \textbf{83.14}    & \textbf{79.77}    & \textbf{75.68}    \\
    \textbf{LLaMA-Adapter}    & \textbf{1.8M}                                & \textbf{85.19}   & \textbf{84.37}    & \textbf{88.30}    & \textbf{84.36}    & \textbf{83.72}    & \textbf{80.32}    & \textbf{86.90}    & \textbf{85.83}    & \textbf{84.05}    \\ \bottomrule
    \end{tabular}%
    % }
    \caption{\textbf{Question Answering Accuracy (\%) on ScienceQA's~\cite{scienceqa} test set.} We report the accuracy of different question classes, including natural science, social science, language science, text context, image context, no context, grades 1-6, and grades 7-12. GPT-3~\cite{brown2020language} of 175B parameters conducts zero-shot answering. LLaMA-Adapter$_T$ and MM-COT$_T$ denote their single-modal variants with text-only input.}
    \vspace{0.1cm}
    \label{tab:scienceqa}
    \end{table*}

==> v1_tables/training_efficiency.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{lrrc}
\toprule
Model         & \makecell[c]{Tuned\\Params} & \makecell[c]{Storage\\Space}  & \makecell[c]{Training\\Time} \\
\cmidrule(lr){1-1} \cmidrule(lr){2-4}
Alpaca~\cite{alpaca}        &   7B             &  13G         &  3 hours  \\
Alpaca-LoRA~\cite{hu2021lora}   &   4.2M          &16.8M   & -          \\
LLaMA-Adapter &\textbf{1.2M} &\textbf{4.7M}   &  \textbf{1 hour}   \\
\bottomrule
\end{tabular}%
}
\caption{\textbf{Efficiency Comparison} of instruction-following methods. The training time is tested on 8 A100 GPUs.}
\label{tab:training_efficiency}
\end{table}

==> v1_tables/zero_init_acc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[t!]
\centering
% \small
\resizebox{0.64\textwidth}{!}{%
\begin{tabular}{l|c}
\toprule
Setting &  Val Acc (\%) \\
\midrule
Rand-Init Attention   & 40.77           \\
Zero-Init Attention   & \textbf{84.04} \\
\textit{\textcolor{blue}{Gain}} &\textcolor{blue}{+43.27}\\
\bottomrule
\end{tabular}%
}
\caption{\textbf{Ablation on Zero-init Attention.}}
\label{tab:zero_init_acc}
\end{table}
